Mata, a Fast and Simple Finite Automata Library (Technical Report)

Mata is a well-engineered automata library written in C++ that offers a unique combination of speed and simplicity. It is meant to serve in applications such as string constraint solving and reasoning about regular expressions, and as a~reference implementation of automata algorithms. Besides basic algorithms for (non)deterministic automata, it implements a fast simulation reduction and antichain-based language inclusion checking. The simplicity allows a straightforward access to the low-level structures, making it relatively easy to extend and modify. Besides the C++ API, the library also implements a Python binding. The library comes with a large benchmark of automata problems collected from relevant applications such as string constraint solving, regular model checking, and reasoning about regular expressions. We show that Mata is on this benchmark significantly faster than all libraries from a wide range of automata libraries we collected. Its usefulness in string constraint solving is demonstrated by the string solver Z3-Noodler, which is based on Mata and outperforms the state of the art in string constraint solving on many standard benchmarks.

==> figs/stats-per-bench-1-swap-bla.tex <==
\begin{tabular}{l ggggg rrrrr gggg rrrr gggg}
\toprule
& \multicolumn{5}{h}{\bincl (136)}       & \multicolumn{5}{c}{\bcsmtlib (386)}   & \multicolumn{4}{h}{\bregexlib (500)}     & \multicolumn{4}{c}{\bpresexpl (170)}   & \multicolumn{4}{h}{\bpressym (170)}   \\\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}\cmidrule(lr){18-21}
& \multicolumn{1}{h}{\textit{TO}} & \multicolumn{1}{h}{\textit{Avg}} & \multicolumn{1}{h}{\textit{Med}} & \multicolumn{1}{h}{\textit{RS}} & \multicolumn{1}{h}{\textit{Std}} & \multicolumn{1}{c}{\textit{TO}} & \multicolumn{1}{c}{\textit{Avg}} & \multicolumn{1}{c}{\textit{Med}} & \multicolumn{1}{c}{\textit{RS}} & \multicolumn{1}{c}{\textit{Std}} & \multicolumn{1}{h}{\textit{TO}} & \multicolumn{1}{h}{\textit{Avg}} & \multicolumn{1}{h}{\textit{Med}} & \multicolumn{1}{h}{\textit{Std}} & \multicolumn{1}{c}{\textit{TO}} & \multicolumn{1}{c}{\textit{Avg}} & \multicolumn{1}{c}{\textit{Med}} & \multicolumn{1}{c}{\textit{Std}} & \multicolumn{1}{h}{\textit{TO}} & \multicolumn{1}{h}{\textit{Avg}} & \multicolumn{1}{h}{\textit{Med}} & \multicolumn{1}{h}{\textit{Std}}\\
\midrule
\rowcolor{GreenYellow}
\mata             &\best 0 & \best{174} & \best 2 & 1\,s & - & \best 0 & \best 1 & \best 1 & 1 & - &\best 0 & \best 1 & \best \nearzero & 9 &\best 0 & 42 & \best 6 & 356 &\best 0 & \best 2 & \best 2 & 6\\
\awali            & 7 & 1\,s & 17 & 3\,s & 27.5 & \best 0 & 6 & 6 & 4 & 3.7 & \best 0 & 46 & 4 & 162 & 6 & \best{21} & 21 & 16 &\best 0 & 8 & 7 & 14\\
\vata             &\best 0 & 324 & 43 & 577 & 1.9 &\best 0 & 7 & 7 & 10 & 4.5 &\best 0 & 42 & 2 & 322 &\best 0 & 121 & 51 & 671 & 1 & 11 & 10 & 11\\
\automatanet      & 9 & 1\,s & 125 & 3\,s & 29.7 &\best 0 & 148 & 153 & 30 & 89.6 &\best 0 & 69 & 66 & 30 &\best 0 & 113 & 117 & 49 & 6 & 103 & 107 & 33\\
\brics            & 5 & 659 & 34 & 2\,s & 17 & 4 & 43 & 43 & 19 & 26.1 & 6 & 103 & 17 & 280 &\best 0 & 66 & 62 & 63 & 6 & 55 & 60 & 33\\
\automatajar      & 10 & 843 & 669 & 1\,s & 21.4 & 7 & 390 & 126 & 3\,s & 236.4 & 48 & 516 & 390 & 521 &\best 0 & 458 & 285 & 1\,s & 6 & 164 & 173 & 52\\
\fado             & 58 & 8\,s & 22\,s & 10\,s & 4840 & 9 & 109 & 112 & 67 & 70.2 & 64 & 6\,s & 1\,s & 11\,s & 1 & 1\,s & 727 & 2\,s & 6 & 135 & 149 & 105\\
\automatapy       & 10 & 913 & 133 & 3\,s & 23.2 & 334 & 24 & TO & 15 & 24.5 & 4 & 520 & 19 & 2\,s & 1 & 372 & 167 & 894 & 6 & 35 & 35 & 25\\
\bottomrule
\end{tabular}


==> figs/stats-per-bench-1.tex <==
 \textbf{benchmark}   & \multicolumn{4}{h}{\textbf{mata}}       & \multicolumn{4}{c}{\textbf{awali}}   & \multicolumn{4}{h}{\textbf{vata}}   & \multicolumn{4}{c}{\textbf{automata.net}}   \\
\midrule
 armc-incl            & 0 & 174 & 2 & 1 s                       & 7 & 1 s & 17 & 3 s                   & 0 & 324 & 43 & 577                  & 9 & 1 s & 125 & 3 s                         \\
 b-smt                & 0 & 1 & 1 & 1                           & 0 & 6 & 6 & 4                        & 0 & 7 & 7 & 10                      & 0 & 148 & 153 & 30                          \\
 email-filter         & 0 & 1 & $\overline{0}$ & 9              & 0 & 46 & 4 & 162                     & 0 & 42 & 2 & 322                    & 0 & 69 & 66 & 30                            \\
 lia-explicit         & 0 & 42 & 6 & 356                        & 6 & 21 & 21 & 16                     & 0 & 121 & 51 & 671                  & 0 & 113 & 117 & 49                          \\
 lia-symbolic         & 0 & 2 & 2 & 6                           & 0 & 8 & 7 & 14                       & 1 & 11 & 10 & 11                    & 6 & 103 & 107 & 33                          \\
 noodler-compl        & 0 & 39 & $\overline{0}$ & 401           & 0 & 73 & 2 & 638                     & 0 & 57 & 2 & 296                    & 0 & 53 & 39 & 110                           \\
 noodler-concat       & 0 & 100 & 10 & 286                      & 0 & 490 & 55 & 1 s                   & \multicolumn{4}{h}{-}               & \multicolumn{4}{c}{-}                       \\
 noodler-inter        & 0 & $\overline{0}$ & $\overline{0}$ & 3 & 6 & 3 & 1 & 7                        & 2 & 4 & $\overline{0}$ & 22         & 0 & 26 & 24 & 9                             \\
 param-inter          & 156 & 1 s & TO & 4 s                    & 157 & 6 s & TO & 7 s                 & 159 & 7 s & TO & 8 s                & 157 & 8 s & TO & 10 s                       \\
 param-union          & 0 & 166 & 7 & 326                       & 0 & 1 s & 81 & 3 s                   & 14 & 6 s & 270 & 12 s               & 0 & 220 & 47 & 314                          \\
\bottomrule

==> figs/stats-per-bench-2.tex <==
 \textbf{benchmark}   & \multicolumn{4}{h}{\textbf{mata}}       & \multicolumn{4}{c}{\textbf{brics}}   & \multicolumn{4}{h}{\textbf{automatalib}}   & \multicolumn{4}{c}{\textbf{fado}}   & \multicolumn{4}{h}{\textbf{automata.py}}   \\
\midrule
 armc-incl            & 0 & 174 & 2 & 1 s                       & 5 & 659 & 34 & 2 s                   & 10 & 843 & 669 & 1 s                       & 58 & 8 s & 22 s & 10 s              & 10 & 913 & 133 & 3 s                       \\
 b-smt                & 0 & 1 & 1 & 1                           & 4 & 43 & 43 & 19                     & 7 & 390 & 126 & 3 s                        & 9 & 109 & 112 & 67                  & 334 & 24 & TO & 15                         \\
 email-filter         & 0 & 1 & $\overline{0}$ & 9              & 6 & 103 & 17 & 280                   & 48 & 516 & 390 & 521                       & 64 & 6 s & 1 s & 11 s               & 4 & 520 & 19 & 2 s                         \\
 lia-explicit         & 0 & 42 & 6 & 356                        & 0 & 66 & 62 & 63                     & 0 & 458 & 285 & 1 s                        & 1 & 1 s & 727 & 2 s                 & 1 & 372 & 167 & 894                        \\
 lia-symbolic         & 0 & 2 & 2 & 6                           & 6 & 55 & 60 & 33                     & 6 & 164 & 173 & 52                         & 6 & 135 & 149 & 105                 & 6 & 35 & 35 & 25                           \\
 noodler-compl        & 0 & 39 & $\overline{0}$ & 401           & 0 & 47 & 8 & 190                     & 0 & 293 & 143 & 793                        & 10 & 646 & 5 & 4 s                  & 3 & 263 & 5 & 2 s                          \\
 noodler-concat       & 0 & 100 & 10 & 286                      & 0 & 136 & 35 & 204                   & \multicolumn{4}{h}{-}                      & 189 & 10 s & 25 s & 13 s            & \multicolumn{4}{h}{-}                      \\
 noodler-inter        & 0 & $\overline{0}$ & $\overline{0}$ & 3 & 0 & 7 & 3 & 21                       & 17 & 276 & 216 & 675                       & 10 & 271 & 52 & 2 s                 & 5 & 38 & 3 & 353                           \\
 param-inter          & 156 & 1 s & TO & 4 s                    & 159 & 6 s & TO & 6 s                 & 227 & 8 s & TO & 13 s                      & 250 & 15 s & TO & 20 s              & 254 & 4 s & TO & 6 s                       \\
 param-union          & 0 & 166 & 7 & 326                       & 0 & 223 & 50 & 307                   & 227 & 10 s & TO & 15 s                     & 115 & 5 s & 12 s & 11 s             & 245 & 11 s & TO & 16 s                     \\
\bottomrule

==> figs/stats-per-bench.tex <==




































\begin{tabular}{llllllllll}
\hline
 bench                 & mata                 & awali                 & vata                 & automata                        \\
\hline                 
 aut\_inclusion        & 0, 175, 2, 1s        & 7, 1067, 18, 13s      & 0, 325, 43, 577      & 9, 845, 61, 14s       \\
 bc\_ere               & 0, 2, 2, 18s         & 0, 6, 6, 19s          & 0, 7, 7, 18s         & 0, 111, 124, 18s       \\
 bc\_inter             & 156, 1.4s, TO, 29s   & 157, 5,8s, TO, 27s    & 159, 6.8s, TO, 26s   & 157, 8.6s, TO, 26s    \\
 bc\_union             & 0, 133, 5, 264       & 0, 1s, 56, 2s         & 14, 3.1s, 153, 14s   & 0, 65, 18, 85         s \\
 email\_filter         & 0, 2, 0, 7           & 0, 48, 5, 165         & 0, 43, 3, 315        & 0, 70, 66, 31           \\
 presburger            & 1, 3, 2, 5s          & 1, 9, 7, 5s           & 2, 12, 10, 6s        & 0, 85, 85, 31           \\
 presburger-explicit   & 0, 104, 6, 880       & 7, 22, 22, 12s        & 0, 206, 52, 1s       & 0, 92, 89, 37             \\
 z3\_noodler           & 8, 39, 0, 6s         & 8, 73, 3, 6s          & 8, 57, 2, 6s         & 8, 47, 32, 6s           \\
 z3\_noodler\_concat   & 0, 101, 11, 287      & 0, 491, 55, 1s        & -                    & -                         \\
 z3\_noodler\_intersect& 4, 1, 0, 4.2s        & 10, 3, 2, 5s          & 6, 5, 0, 4s          & 0, 22, 23, 4s           \\
\hline
 bench                 & brics                & (j)alib              & fado                    & (py)alib             \\
\hline
 aut\_inclusion        & 5, 660, 35, 11s    & 5, 41, 38, 11s     & 58, 8.4s, 22s, 27s  & 10, 460, 68, 16s   \\
 bc\_ere               & 4, 41, 41, 19s     & 8, 243, 57, 19s    & 9, 45, 41, 20s       & 334, 8, TO, 10s    \\
 bc\_inter             & 159, 5.8s, TO, 27s & 227, 2.3s, TO, 21s & 250, 15s, TO, 12s   & 253, 5.7s, TO, 12s \\
 bc\_union             & 0, 0, 0, 0         & 226, 3, TO, 22s    & 115, 858, 1.5s, 29s   & 242, 9.6s, TO, 15s \\
 email\_filter         & 0, 101, 17, 280    & 46, 151, 111, 17s  & 66, 5.3s, 1.3s, 21s   & 4, 319, 14, 5s     \\
 presburger            & 7, 56, 61, 12s     & 7, 30, 27, 12s     & 7, 72, 79, 12s        & 7, 19, 19, 12s     \\
 presburger-explicit   & 0, 70, 62, 78      & 0, 54, 49, 25        & 2, 651, 395, 7s       & 1, 471, 88, 6s     \\
 z3\_noodler           & 8, 48, 9, 6s       & 8, 65, 50, 6s      & 8, 551, 4, 7s         & 1, 237, 4, 3s      \\
 z3\_noodler\_concat   & 0, 137, 35, 205    & -                    & 189, 9.7s, 25s, 27s & -                    \\
 z3\_noodler\_intersect& 0, 8, 4, 45        & 21, 76, 68, 4s     & 14, 271, 52, 4s      & 9, 31, 3, 26s       \\
\hline
\end{tabular}


%  & mona         
%                 
%& 41, 7, 4, 27s  
%& -              
%& -              
%& -              
%& -              
%& 32, 1, 1, 23s  
%& -              
%& -              
%& -              
%& -              


==> figs/stats-per-op-1.tex <==
 \textbf{operation}   & \multicolumn{3}{h}{\textbf{mata}}   & \multicolumn{3}{c}{\textbf{awali}}   & \multicolumn{3}{h}{\textbf{vata}}   & \multicolumn{3}{c}{\textbf{automata.net}}        \\
\midrule
 complement           & 25 & 1 & 315                        & 38 & 2 & 462                         & 36 & 3 & 294                        & 73 & 59 & 89                                     \\
 concatenation        & 78 & 8 & 235                        & 166 & 22 & 402                       & \multicolumn{3}{h}{-}               & \multicolumn{3}{c}{-}                            \\
 emptiness            & $\overline{0}$ & $\overline{0}$ & 2 & 17 & $\overline{0}$ & 138            & 14 & $\overline{0}$ & 130           & $\overline{0}$ & $\overline{0}$ & $\overline{0}$ \\
 inclusion            & 37 & $\overline{0}$ & 576           & 250 & 2 & 2 s                        & 85 & 1 & 374                        & 245 & 43 & 1 s                                   \\
 intersection         & 295 & $\overline{0}$ & 3 s          & 312 & $\overline{0}$ & 2 s           & 699 & $\overline{0}$ & 4 s          & 621 & 14 & 4 s                                   \\
 trim                 & 76 & $\overline{0}$ & 828           & 516 & $\overline{0}$ & 4 s           & 408 & $\overline{0}$ & 3 s          & 31 & 9 & 165                                     \\
 union                & 14 & $\overline{0}$ & 45            & 173 & $\overline{0}$ & 527           & 2 s & $\overline{0}$ & 5 s          & 69 & 6 & 163                                     \\
\bottomrule

==> figs/stats-per-op-2.tex <==
 \textbf{operation}   & \multicolumn{3}{h}{\textbf{mata}}   & \multicolumn{3}{c}{\textbf{brics}}               & \multicolumn{3}{h}{\textbf{automatalib}}   & \multicolumn{3}{c}{\textbf{fado}}   & \multicolumn{3}{h}{\textbf{automata.py}}   \\
\midrule
 complement           & 25 & 1 & 315                        & 46 & 24 & 140                                    & 75 & 31 & 657                              & 320 & 3 & 2 s                       & 226 & 25 & 2 s                             \\
 concatenation        & 78 & 8 & 235                        & 136 & 35 & 204                                   & \multicolumn{3}{h}{-}                      & 6 s & 10 s & 10 s                   & \multicolumn{3}{h}{-}                      \\
 emptiness            & $\overline{0}$ & $\overline{0}$ & 2 & $\overline{0}$ & $\overline{0}$ & $\overline{0}$ & 3 & 2 & 5                                  & 223 & $\overline{0}$ & 2 s          & 53 & $\overline{0}$ & 1 s                  \\
 inclusion            & 37 & $\overline{0}$ & 576           & 204 & 10 & 1 s                                   & 60 & 42 & 102                              & 3 s & 84 & 8 s                      & 263 & 6 & 1 s                              \\
 intersection         & 295 & $\overline{0}$ & 3 s          & 115 & 4 & 1 s                                    & 91 & 59 & 748                              & 479 & 48 & 3 s                      & 39 & 2 & 479                               \\
 trim                 & 76 & $\overline{0}$ & 828           & \multicolumn{3}{c}{-}                            & \multicolumn{3}{h}{-}                      & 10 & 3 & 70                         & \multicolumn{3}{h}{-}                      \\
 union                & 14 & $\overline{0}$ & 45            & 99 & 2 & 232                                     & 311 & 2 & 3 s                              & 1 s & 84 & 6 s                      & 203 & TO & 377                             \\
\bottomrule

==> figs/stats-per-op.tex <==
\begin{tabular}{llllllllll}
\hline
 op                  & mata         & awali       & vata         & automata           \\
\hline
 complement          & 33, 1, 10s   & 39, 2, 11s  & 46, 4, 10s   & 60, 53, 10s      \\
 concatenation       & 79, 9, 236   & 166, 22, 402& -            & -                  \\
 emptiness           & 0, 0, 9s     & 17, 0, 9s   & 14, 0, 9s    & 0, 0, 9s         \\
 inclusion           & 38, 0, 576   & 251, 3, 6s  & 85, 2, 372   & 204, 41, 7s      \\
 intersection        & 296, 0, 8s   & 312, 1, 5s  & 699, 0, 6s   & 642, 14, 5s      \\
 trim                & 76, 0, 7s    & 516, 1, 6s  & 409, 0, 5s   & 31, 9, 1s          \\
 union               & 15, 0, 15s   & 174, 0, 15s & 1614, 1, 15s & 66, 6, 15s       \\
\hline
 op                  & brics          & (j)alib         & fado            & (py)alib          \\
\hline
 complement          & 47, 25, 11s    & 72, 33, 11s     & 320, 3, 12s     & 237, 25, 26s    \\
 concatenation       & 137, 35, 205   & -               & 5.6s, 9.5s, 27s & -                 \\
 emptiness           & 0, 0, 9s       & 3, 2, 13s       & 224, 0, 16s     & 54, 0, 18s      \\
 inclusion           & 203, 10, 5s    & 51, 35, 16s     & 3.1s, 89, 23s   & 268, 7, 8s      \\
 intersection        & 116, 4, 9s     & 99, 64, 11s     & 458, 48, 14s    & 39, 2, 17s      \\
 trim                & -              & -               & 11, 4, 16s      & -                 \\
 union               & 100, 3, 15s    & 274, 2, 28s     & 1.3s, 84, 26s   & 203, TO, 13s    \\
\hline
\end{tabular}





%& mona            
%                  
%& 1, 1, 23s       
%& -               
%& 0, 0, 23s       
%& 7, 4, 27s       
%& -               
%& -               
%& -               


==> figs/stats-relative.tex <==
 bench          &   mata &   mata-sim &   awali & vata   & automata.net   &   brics & automatalib   &    fado & automata.py   \\
\midrule
 armc-incl      &      1 &       1.28 &   27.52 & 1.86   & 29.73          &   16.98 & 21.44         & 4839.55 & 23.22         \\
 b-smt          &      1 &       1.39 &    3.7  & 4.52   & 89.64          &   26.13 & 236.36        &   70.16 & 24.47         \\
 email-filter   &      1 &      32.37 &   25.07 & 22.59  & 37.19          &   55.3  & 273.35        & 9999.29 & 282.41        \\
 lia-explicit   &      1 &       0.58 &    2.22 & 2.88   & 2.69           &    1.57 & 10.89         &   85.17 & 25.38         \\
 lia-symbolic   &      1 &       0.99 &    3.46 & 4.65   & 51.82          &   27.99 & 82.47         &   67.54 & 17.97         \\
 noodler-compl  &      1 &       1.6  &    1.85 & 1.45   & 1.37           &    1.22 & 7.44          &  137.53 & 15.58         \\
 noodler-concat &      1 &       4    &    4.87 & -      & -              &    1.36 & -             & 1979.56 & -             \\
 noodler-inter  &      1 &      30.84 &    4.02 & 6.42   & 33.98          &    9.04 & 371.23        &  363.49 & 51.51         \\
 param-inter    &      1 &       0.67 &    5.36 & 7.3    & 7.27           &    6.49 & 1.43          & 2148.64 & 58.85         \\
 param-union    &      1 &       1.09 &    8.61 & 51.77  & 1.33           &    1.34 & 833.69        & 1618.04 & 5860.62       \\
\bottomrule
